Digital signatures with classical shadows on near-term quantum computers

Quantum mechanics provides cryptographic primitives whose security is grounded in hardness assumptions independent of those underlying classical cryptography. However, existing proposals require low-noise quantum communication and long-lived quantum memory, capabilities which remain challenging to realize in practice. In this work, we introduce a quantum digital signature scheme that operates with only classical communication, using the classical shadows of states produced by random circuits as public keys. We provide theoretical and numerical evidence supporting the conjectured hardness of learning the private key (the circuit) from the public key (the shadow). A key technical ingredient enabling our scheme is an improved state-certification primitive that achieves higher noise tolerance and lower sample complexity than prior methods. We realize this certification by designing a high-rate error-detecting code tailored to our random-circuit ensemble and experimentally generating shadows for 32-qubit states using circuits with $\geq 80$ logical ($\geq 582$ physical) two-qubit gates, attaining 0.90 $\pm$ 0.01 fidelity. With increased number of measurement samples, our hardware-demonstrated primitives realize a proof-of-principle quantum digital signature, demonstrating the near-term feasibility of our scheme.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> new_shadow.tex <==
\newpage
\section{Shadow overlap protocols \ml{This section is backed up in shadow.tex}}\label{sec:shadow}
In Theorem~\ref{thm:noiseless_single_bit_security}, we show that any shadow-overlap-type state certification protocol can be adapted into a digital signature scheme. While known schemes for shadows-based state certification all have sample complexity (size of shadows) that are nominally polynomial, for a practical application, it is desirable to make the exact, numeric size of shadows small, given the attributes of available quantum hardware. The goal of this section is to provide a shadow-based certification protocol which improves on known methods. We begin by briefly summarizing the relevant aspects of the protocol of Ref.~\cite{huang2024certifying}, before introducing the improved protocol. Interested reader is encouraged to see Ref.~\cite{huang2024certifying} for additional details.

On a high level, the procedure for certifying that a ``lab'' state $\rho$ is close to some target state $\ket{\psi}$  of Protocol 2 of \cite{huang2024certifying} is as follows. To generate the shadows, we randomly select a subset of $r$ qubits to measure the lab state in a random single-qubit Pauli basis and measure the rest in the computational basis. Using the shadows, compute the overlap with some operator dependent on the target quantum state to certify. Specifically, the procedure yields the so-called shadow overlap estimator $\omega$, which also satisfies $\mathbb{E}[\omega]=\mathrm{tr}(L\rho)$ where $L$ is some operator and $\rho$ is the measured state. Given $L$, one can identify the certification procedure.

The procedure for certifying quantum state fidelity in \cite{huang2024certifying} uses an $L$ such that $\vert\psi\rangle$ is an eigenvector with eigenvalue $1$ and that the shadow overlap protocol over shadows generated from state $\rho$ yields $\mathrm{tr}(L\rho)$ in expectation (i.e., $\mathrm{tr}(L\rho)=\mathbb{E}[\omega]$, where $\omega$ is the computed shadow overlap for a given trial). A step in establishing $\text{tr}(L\rho)=\mathbb{E}[\omega]$ is that $L$ can be written as the sum
\begin{align}
L=\frac{1}{N}\sum_{r\in[m]}\sum_{k=\{k_1,\dots,k_r\}}\sum_{z_k\in\{0,1\}^{n-r}}\vert z_k\rangle\langle z_k\vert\otimes L_{z_k}\label{eqn:L_form},
\end{align}
where $m$ is a positive integer that is at most $n$, $k$ is a subset of $r$ out of $n$ qubits, $z_k$ corresponds to a particular measurement outcome on the qubits measured in the fixed $Z$ basis, $L_{z_k}$ is efficiently computable, and $N$ is the number of terms due to the summation over $r$ and $k$ which is given by $\sum_{k=1}^m\binom{n}{k}$. 
Specifically, \cite{huang2020predicting} uses the following definition of $L_{z_k}$:
\begin{align}
L_{z_k}=\sum_{\substack{\ell_1,\ell_2\in\{0,1\}^r\\\mathrm{dist}(\ell_1,\ell_2)=r}}\vert\Psi_{z_k}^{\ell_1,\ell_2}\rangle\langle\Psi_{z_k}^{\ell_1,\ell_2}\vert\quad\text{with}\quad\vert\Psi_{z_k}^{\ell_1,\ell_2}\rangle=\frac{\Psi(z_k^{(\ell_1)})\vert\ell_1\rangle+\Psi(z_k^{(\ell_2)})\vert\ell_2\rangle}{\sqrt{\vert\Psi(z_k^{(\ell_1)})\vert^2+\vert\Psi(z_k^{(\ell_2)})\vert^2}},
\end{align}
where $\Psi$ is a model providing query access to amplitudes of $\ket{\psi}$, $z_k^{\ell}$ equals $\ell$ on bits $k_1,\dots,k_r$ and equals $z_k$ on the remaining $n-r$ bits.

To certify a state, $T$ copies of the state $\rho$ are measured according to the shadow overlap protocol and produce an estimator $\hat{\omega}$, which is given by the empirical average $\frac{1}{T}\sum_{t=1}^T \omega_t$. Ref.~\cite{huang2024certifying} states that $T=O(2^{2m})$ samples are required such that $\vert\hat{\omega}-\mathbb{E}[\omega]\vert\leq\varepsilon$ with high probability. The number of samples required (adjusting for an error in the use of Hoeffding's inequality in \cite{huang2020predicting}) is given by the following theorem: 
\begin{theorem}[Theorem 5 of \cite{huang2024certifying}, corrected]\label{thm:fixed_huang_verification}
Using $T\geq\frac{2^{4m-1}}{\varepsilon^2}\ln\frac{2}{\delta}$ samples of the state $\rho$, the empirical average $\frac{1}{T}\sum_{t=1}^T\omega_t$ computed by Protocol 2 of \cite{huang2024certifying} is within $\varepsilon$ additive distance from the shadow overlap $\mathbb{E}[\omega]$ with probability at least $1-\delta$.
\end{theorem}
\begin{proof}
The proof is identical to Theorem 5 of \cite{huang2020predicting} except for the application of Hoeffding's inequality. Instead of Eq. 30 of \cite{huang2024certifying}, the corrected quantity is
\begin{align}
\Pr\left[\left\vert\frac{1}{T}\sum_{t=1}^T\omega_t-\mathbb{E}[\omega]\right\vert>\varepsilon\right]\leq2e^{-\frac{2T^2\varepsilon^2}{T(2^{2m-1}-(-2^{2m-1}))^2}}=2e^{-\frac{T\varepsilon^2}{2^{4m-1}}}\leq\delta.
\end{align}
Solving for $T$ completes the proof.
\end{proof}
While this determines the sample complexity required to estimate the shadow overlap $\omega$ precisely, it still remains to show the connection between $\mathbb{E}[\omega]$ and the fidelity $\langle\psi\vert\rho\vert\psi\rangle$, which is necessary for certification. For any $L$, one can compute the so-called relaxation time $\tau$, which corresponds to the relaxation time of the Markov chain defined by $L$. Then, Theorem 4 of \cite{huang2024certifying} guarantees a equivalence between shadow overlap and fidelity.  Namely, if $\mathbb{E}[\omega]\geq 1-\varepsilon$, then $\langle\psi\vert\rho\vert\psi\rangle\geq1-\tau\varepsilon$ (high shadow overlap implies high fidelity). Conversely, if $\langle\psi\vert\rho\vert\psi\rangle\geq 1-\varepsilon$, then $\mathbb{E}[\omega]\geq 1-\varepsilon$ (high fidelity implies high shadow overlap).

For a concrete experiment, it becomes important to determine $\tau$. The relaxation time $\tau$ for $m=1$ is shown to be upper-bounded by $n^2$ for Haar random states. For noisy quantum devices, however, even if $\rho$ is prepared by executing the quantum circuit for $\vert\psi\rangle$, $\langle\psi\vert\rho\vert\psi\rangle$ cannot be arbitrarily close to 1 due to the fidelity limitations of the device. Having $\langle\psi\vert\rho\vert\psi\rangle\geq1-\varepsilon$, where $\varepsilon$ is the infidelity, implies $\mathbb{E}[\omega]\geq 1-\varepsilon$, which certifies that $\langle\psi\vert\rho\vert\psi\rangle\geq1-\tau\varepsilon$. This means the infidelity of certification grows by a factor of $\tau$. For $\tau=O(n^2)$, certification becomes impossible for low fidelity devices as the requirement $\tau\epsilon\ll 1$ implies $\epsilon\ll\frac{1}{O(n^2)}$.  Although empirical evidence in Fig.~\ref{fig:relaxation_time}\textbf{a} suggests $\tau=O(n)$ for Haar-random states, this is still highly impractical for fidelities below $0.99$.

Specifically, to see this issue, we can state the corrected shadow overlap protocol sample complexity for obtaining completeness and soundness of certification.
\begin{theorem}[Theorem 6 of \cite{huang2024certifying}, corrected]\label{thm:fixed_huang_verification_completeness_and_soundness}
Given any $n$-qubit hypothesis state $\vert\psi\rangle$ with a relaxation time $\tau\geq 1$, error $\varepsilon>0$, failure probability $\delta>0$, and
\begin{align}
T=2^{4m+3}\cdot\frac{\tau^2}{\varepsilon^2}\cdot\ln\frac{2}{\delta}
\label{eq:original-sample-complexity}
\end{align}
samples of an unknown $n$-qubit state $\rho$, with probability at least $1-\delta$, Protocol \ref{prot:random_clifford_improved} with shadow overlap threshold $\omega_{\mathrm{threshold}}\equiv1-\varepsilon'=\frac{3\varepsilon}{4\tau}$ will correctly output \textsc{Failed} if the fidelity is low, i.e. $\langle\psi\vert\rho\vert\psi\rangle<1-\varepsilon$, and will correctly output \textsc{Certified} if the fidelity is high, i.e. $\langle\psi\vert\rho\vert\psi\rangle\geq1-\frac{\varepsilon}{2\tau}$.
\end{theorem}
\begin{proof}
The proof is identical to Theorem 6 of \cite{huang2024certifying} except we use Theorem \ref{thm:fixed_huang_verification}. Simply substituting $\varepsilon\rightarrow\varepsilon/\tau-\varepsilon'=\frac{\varepsilon}{4\tau}$.
\end{proof}

\subsection{Improved random Pauli shadow overlap protocols}\label{sec:supp_improved_shadow}
One way of reducing the sample complexity (Eq.~\ref{eq:original-sample-complexity}) is by reducing the relaxation time $\tau$. In order to do so, we make two observations. First, increasing the level $m$ of the protocol increases the connectivity of the Markov chain. This is apparent since the supported edges are between bitstrings that differ in at most $m$ bits. Second, as long as $L_{z_k}$ is the outer product of normalized quantum states, any $L$ of the form of Eq.~\ref{eqn:L_form} has a correspondence to a shadow overlap procedure, with $L_{z_k}$ as the observable of interest.

As a result, we define the following operator
\begin{align}
L=\binom{n}{m}^{-1}\times\sum_{k=\{k_1,\dots,k_m\}}\sum_{z_k\in\{0,1\}^{n-m}}\vert z_k\rangle\langle z_k\vert\otimes L_{z_k}, \qquad \text{with } \quad L_{z_k}=\vert\Psi_{z_k}\rangle\langle\Psi_{z_k}\vert\quad\text{and}\quad\vert\Psi_{z_k}\rangle=\frac{\sum_{\ell\in\{0,1\}^m}\Psi(z_k^\ell)\vert\ell\rangle}{\sqrt{\sum_{\ell\in\{0,1\}^m}\vert\Psi(z_k^\ell)\vert^2}}.
\end{align}
Now, we redefine the shadow overlap procedure with the new $L_{z_k}$. The same steps of Proposition 3 of \cite{huang2024certifying} yield $\mathrm{tr}[L\rho]=\mathbb{E}[\omega]$.

We will prove later that $L\vert\psi\rangle=\vert\psi\rangle$. It is clear from definition that $L$ is Hermitian. One also can define the Markov chain with transition matrix $P=S^{-1/2}F^\dagger LFS^{1/2}$, which is exactly the same as Proposition 3 of \cite{huang2024certifying}, which allows us to compute the relaxation time and bound the fidelity from the shadow overlap.

Fig.~\ref{fig:relaxation_time} shows the relaxation of Haar random states and states prepared by the ansatz of our experimental quantum circuits using different definitions of the operator $L$. In particular, our experimental quantum circuit ansatz is as described in the main text, and we show the shadow overlap of those with two blocks and $\lceil\log_2n\rceil$ layers. We observe in Fig.~\ref{fig:relaxation_time}\textbf{a} that for Protocol 2 of \cite{huang2020predicting}, increasing $m$ does not reduce the relaxation time meaningfully beyond $m=3$. Additionally, the slopes seem to be about the same for different values of $m$, indicating similar asymptotic scaling of $\tau$. On the other hand, Fig.~\ref{fig:relaxation_time}\textbf{b} shows that our protocol achieves a notably lower relaxation time. For $m=4$, extrapolating to $n=32$ gives $\tau\approx 8$. Note that the horizontal axis scaling is different from Fig.~\ref{fig:relaxation_time}\textbf{a}. The asymptotic scaling also improves with $m$. An overall trend is that increasing $m$ or $n$ decreases the variance in the relaxation time. We also show that the choice of the quantum circuits we make does not impact the average relaxation time very much, as is evidenced by Fig.~\ref{fig:relaxation_time}\textbf{c}, but it does increase the variance in the relaxation time.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\linewidth]{imgs/relaxation_time_figure.pdf}
    \caption{\textbf{Relaxation time of the certification procedures. a}, Relaxation time of Protocol 2 of \cite{huang2024certifying} for Haar random states. \textbf{b}, Relaxation time of our Protocol \ref{prot:random_pauli_improved} for Haar random states. \textbf{c}, Relaxation time of our $m=4$ protocol for Haar random states and the state generated using the ansatz of our experimental quantum circuits with two blocks and $\lceil\log_2n\rceil$ layers. Error bars show the standard deviation. Data points with $n\leq12$ are averaged over 10 random instances, whereas each data point beyond that only consists of a single instance.}
    \label{fig:relaxation_time}
\end{figure}

To understand why this construction achieves a lower relaxation time, consider the extreme case of $L=\vert\psi\rangle\langle\psi\vert$. All eigenvectors other than $\vert\psi\rangle$ has eigenvalue zero and the relaxation time is the smallest it can be, i.e. $\tau=1$. The operator $L$ defined in \cite{huang2024certifying} is not $\vert\psi\rangle\langle\psi\vert$ even for $m=n$. This is due to the normalization factors of $\vert\Psi_{z_k}^{\ell_1,\ell_2}\rangle$ being the root of the sum of two probabilities always. On the other hand, for $m=n$, our $L$ operator is exactly $\vert\psi\rangle\langle\psi\vert$.

Additionally, this construction of $L$ is more natural than the scheme in \cite{huang2024certifying}. Specifically, $L_{z_k}$ is the collapsed state of the hypothesis state $\vert\psi\rangle$ conditioned on the qubits not in $k$ being measured to $z_k$. Although $L$ is a sum of these collapsed states, it is not $\vert\psi\rangle\langle\psi\vert$ even up to normalization. It may be tempting to interpret $L$ as $\vert\psi\rangle$ going through a random measurement channel up to some normalization, but even this is not correct since each term corresponding to $z_k$ have equal weight instead of proportional to the measurement probability. In fact, if we use the density operator of $\vert\psi\rangle$ going through a random measurement channel, it would not have $\vert\psi\rangle$ as an eigenvector in general.

We now formally describe the protocol in Protocol \ref{prot:random_pauli_improved} and prove its correctness.



\parbox{0.96\textwidth}{\begin{protocol_framed}[Improved level-$m$ shadow overlap]\label{prot:random_pauli_improved}\quad 
\normalfont
\newline
\begin{flushleft}\underline{Input:}\end{flushleft}
 \vspace{-1.5em}
 \begin{itemize}
    \item $T$ samples of an unknown state $\rho$.
    \item A model $\Psi$ that gives query access to the amplitudes of $\vert\psi\rangle$.
    \item A level $m\in[n]$.
    \item Error $0\leq\varepsilon'<1$, or equivalently shadow overlap threshold $\omega_{\mathrm{threshold}}\equiv1-\varepsilon'
    $.
\end{itemize}
\begin{flushleft}\underline{Procedure:}\end{flushleft}
 \vspace{-1.5em}
 \begin{enumerate}
    \item Uniformly choose $m$ random qubits denoted by $k=\{k_1,\dots,k_m\}$.
    \item Perform single-qubit $Z$-basis measurements on all but qubits $k_1,\dots,k_m$ of $\rho$. Denote the measurement outcomes collectively by $z_k\in\{0,1\}^{n-m}$.
    \item For each qubit $k_1,\dots,k_m$, choose an $X,Y,Z$-basis measurement uniformly at random and measure it. Denote the post-measurement state of these qubits by $\vert s_1\rangle,\dots,\vert s_m\rangle$. Compute the classical shadow
    \begin{align}
        \sigma=(3\vert s_1\rangle\langle s_1\vert-\mathbb{I})\otimes\cdots\otimes(3\vert s_m\rangle\langle s_m\vert-\mathbb{I}).\label{eqn:pauli_shadow}
    \end{align}
    \item Query the model $\Psi$ for all choices of $m$-bit strings $\ell$ to obtain the normalized state
    \begin{align}
        \vert\Psi_{z_k}\rangle=\frac{\sum_{\ell\in\{0,1\}^m}\Psi(z_k^\ell)\vert\ell\rangle}{\sqrt{\sum_{\ell\in\{0,1\}^m}\vert\Psi(z_k^\ell)\vert^2}},
    \end{align}
    where $z_k^{\ell}$ equals $\ell$ on bits $k_1,\dots,k_m$ and equals $z_k$ on the remaining $n-m$ bits.
    \item Compute the overlap
    \begin{align}
        \omega=\mathrm{tr}(L_{z_k}\sigma)\quad\text{with}\quad L_{z_k}=\vert\Psi_{z_k}\rangle\langle\Psi_{z_k}\vert.
    \end{align}
    \item Repeat steps 1 to 5 for $T$ times to obtain overlaps $\omega_1,\dots,\omega_T$. Report the estimated shadow overlap
    \begin{align}
        \hat{\omega}=\frac{1}{T}\sum_{t=1}^T\omega_t.
    \end{align}
    \item If the estimated shadow overlap $\hat{\omega}\geq 1-\varepsilon'$, output \textsc{Certified}. Otherwise, output \textsc{Failed}.
\end{enumerate}
\end{protocol_framed}}

\begin{lemma}\label{lem:eigenvector}
Consider a quantum state $\psi$
\begin{align}
\vert\psi\rangle=\Psi(z)\vert z\rangle.
\end{align}
Define an operator $L$
\begin{align}
L=\binom{n}{m}^{-1}\times\sum_{k=\{k_1,\dots,k_m\}}\sum_{z_k\in\{0,1\}^{n-m}}\vert z_k\rangle\langle z_k\vert\otimes L_{z_k},
\end{align}
where
\begin{align}
L_{z_k}=\vert\Psi_{z_k}\rangle\langle\Psi_{z_k}\vert\quad\text{with}\quad\vert\Psi_{z_k}\rangle=\frac{\sum_{\ell\in\{0,1\}^m}\Psi(z_k^\ell)\vert\ell\rangle}{\sqrt{\sum_{\ell\in\{0,1\}^m}\vert\Psi(z_k^\ell)\vert^2}},
\end{align}
where $z_k^{\ell}$ equals $\ell$ on bits $k_1,\dots,k_m$ and equals $z_k$ on the remaining $n-m$ bits. We have \begin{align}
L\vert\psi\rangle=\vert\psi\rangle.
\end{align}
\end{lemma}
\begin{proof}
We first observe that given $m$ qubits specified by vector $k$,
\begin{align}
\langle z_k\vert\psi\rangle=\langle z_k\vert\sum_z\Psi(z)\vert z\rangle=\langle z_k\vert\sum_{z_k'}\sum_{\ell\in\{0,1\}^m}\Psi(z_k'^\ell)\vert z_k'\rangle\otimes\vert\ell\rangle_k=\sum_{\ell\in\{0,1\}^m}\Psi(z_k^\ell)\vert\ell\rangle_k,
\end{align}
which means that the post selected state is
\begin{align}
\frac{\langle z_k\vert\psi\rangle}{\sqrt{\langle\psi\vert z_k\rangle\langle z_k\vert\psi\rangle}}=\vert\Psi_{z_k}\rangle\quad
\end{align}
for $\vert\Psi_{z_k}\rangle$ and $L_{z_k}$ defined in the lemma. Additionally,
\begin{align}
\vert\psi\rangle=\mathbb{I}\vert\psi\rangle=\sum_{z_k}\vert z_k\rangle\langle z_k\vert\psi\rangle=\sum_{z_k}\vert z_k\rangle\otimes\sum_{\ell\in\{0,1\}^m}\Psi(z_k^\ell)\vert\ell\rangle_k=\sum_{z_k}\sqrt{p(z_k)}\vert z_k\rangle\otimes\vert\Psi_{z_k}\rangle,
\end{align}
where $p(z_k)=\sum_{\ell\in\{0,1\}^m}\vert\Psi(z_k^\ell)\vert^2$.
\begin{align}
\binom{n}{m}L\vert\psi\rangle
=&\sum_{k}\sum_{z_k}\vert z_k\rangle\langle z_k\vert\otimes L_{z_k}\vert\psi\rangle\\
=&\sum_{k}\sum_{z_k}\left(\vert z_k\rangle\otimes\vert\Psi_{z_k}\rangle_k\right)\left(\langle z_k\vert\otimes\langle\Psi_{z_k}\vert_k\right)\sum_{z_k'}\sqrt{p(z_k')}\vert z_k'\rangle\otimes\vert\Psi_{z_k'}\rangle\\
=&\sum_{k}\sum_{z_k}\sqrt{p(z_k)}\vert z_k\rangle\otimes\vert\Psi_{z_k}\rangle_k =\sum_{k}\vert\psi\rangle=\binom{n}{m}\vert\psi\rangle.
\end{align}
\end{proof}

\begin{lemma}\label{lem:trace_equal_shadow_overlap_pauli}
For $\omega$ of Protocol \ref{prot:random_pauli_improved}, we have
\begin{align}
\mathrm{tr}(L\rho)=\mathbb{E}[\omega].
\end{align}
\end{lemma}
\begin{proof}
We follow the same idea as Proposition 3 of \cite{huang2024certifying}.
\begin{align}
\mathrm{tr}[L\rho]&=\binom{n}{m}^{-1}\times\sum_{k=\{k_1,\dots,k_m\}}\sum_{z_k\in\{0,1\}^{n-m}}\mathrm{tr}\left(\langle z_k\vert\rho\vert z_k\rangle\right)\cdot \mathrm{tr}\left(L_{z_k}\cdot\frac{\langle z_k\vert\rho\vert z_k\rangle}{\mathrm{tr}(\langle z_k\vert\rho\vert z_k\rangle)}\right)=\underset{k,z_k}{\mathbb{E}}\mathrm{tr}\left(L_{z_k}\cdot\frac{\langle z_k\vert\rho\vert z_k\rangle}{\mathrm{tr}(\langle z_k\vert\rho\vert z_k\rangle)}\right).
\end{align}
We note that converting the sum into expectation is valid just like in \cite{huang2020predicting}, although the sampling process is different. In \cite{huang2020predicting}, the procedure samples $r$, followed by sampling $k=\{k_1,\dots,k_r\}$, and finally measuring $z_k$. Here, we directly sample $k=\{k_1,\dots,k_m\}$ and then measure $z_k$. Following the rest of the steps identically as \cite{huang2024certifying} completes the proof.
\end{proof}

\begin{theorem}\label{thm:shadow_implies_fidelity_pauli}
Let $\lambda_1=1-\frac{1}{\tau}$ be the second largest eigenvalue of the transition matrix $P$ defined as $P=S^{-1/2}F^\dagger LFS^{1/2}$ for state $\vert\psi\rangle$, where $L$ is as defined in Lemma \ref{lem:eigenvector}. The shadow overlap satisfies the following. If $\mathbb{E}[\omega]\geq 1-\varepsilon$, then $\langle\psi\vert\rho\vert\psi\rangle\geq 1 - \tau\varepsilon$. If $\langle\psi\vert\rho\vert\psi\rangle\geq 1-\varepsilon$, then $\mathbb{E}[\omega]\geq 1-\varepsilon$ for $\omega$ as defined in Protocol \ref{prot:random_pauli_improved}.
\end{theorem}
\begin{proof}
The proof is identical to Theorem 4 of \cite{huang2024certifying}.
\end{proof}

\begin{theorem}\label{thm:random_pauli_verification}
Using $T=2^{2m+1}\cdot\frac{1}{\varepsilon^2}\cdot\ln(\frac{2}{\delta})$ samples of the state $\rho$, the empirical average $\frac{1}{T}\sum_{t=1}^T\omega_t$ computed by Protocol \ref{prot:random_pauli_improved} is within $\varepsilon$ additive distance from the shadow overlap $\mathbb{E}[\omega]$ with probability at least $1-\delta$.
\end{theorem}
\begin{proof}
Since $L_{z_k}$ is the outer product of one normalized vector, $\|L_{z_k}\|_1=1$. Following the rest of proof identically as Theorem \ref{thm:fixed_huang_verification} while noting the difference in $\|L_{z_k}\|_1=1$ instead of $\|L_{z_k}\|_1\leq2^{m-1}$ completes the proof.
\end{proof}

To reduce the relaxation time $\tau$, we want $m$ to be as high as possible. However, the sample complexity required so that the estimator of the shadow overlap is close to the expectation value is $O(2^{2m})$ as stated in Theorem \ref{thm:random_pauli_verification}. Nevertheless, compared the protocol in \cite{huang2024certifying} where the sample complexity is proportional to $2^{4m-1}$, we need quadratically fewer samples in $m$.

\subsection{Random Clifford shadow overlap protocols}

Nevertheless, for large $m$, even $2^{2m}$ samples can be an obstacle in practice. Fortunately, the shadow overlap variance bound can be notably improved if the shadows are obtained using random Clifford measurements. For any observable $O$ and set $\hat{o}=\mathrm{tr}(O\hat{\rho})$, where $\hat{\rho}$ is a classical shadow, we have
\begin{align}
\mathrm{Var}[\hat{o}]\leq\left\|O-\frac{\mathrm{tr}(O)}{2^n}\mathbb{I}\right\|^2_{\mathrm{shadow}}=\|O_0\|^2_{\mathrm{shadow}}
\end{align}
from Lemma 1 of \cite{huang2020predicting}, where the second equality serves as a definition for $O_0$ which is a traceless operator in $\mathbb{H}_{2^n}$. For classical shadows obtained by random Clifford measurements, we have
\begin{align}
\|O_0\|_{\mathrm{shadow}}^2\leq3\mathrm{tr}(O^2)
\end{align}
by Proposition 1 of \cite{huang2020predicting}. Since our operator $L_{z_k}$ is an outer product of a normalized vector,
\begin{align}
\mathrm{Var}[\omega_{z_k}]\leq\left\|L_{z_k}-\frac{\mathrm{tr}(L_{z_k})}{2^n}\mathbb{I}\right\|_{\mathrm{shadow}}\leq3,
\end{align}
where $\omega_{z_k}$ is the shadow overlap for the measurement outcome $z_k$ on the $n-m$ qubits other than those specified by set $k$.

It should be noted that the above is the variance of $\omega_{z_k}$, not $\omega$. Each $\omega_{z_k}$ could have variation in the expectation value between $0$ and $1$. This is because
\begin{align}
\mathbb{E}[\omega_{z_k}]=\underset{\mathrm{shadows}~\sigma}{\mathbb{E}}[\mathrm{tr}(L_{z_k}\sigma)]=\mathrm{tr}\left(L_{z_k}\cdot\frac{\langle z_k\vert\rho\vert z_k\rangle}{\mathrm{tr}(\langle z_k\vert\rho\vert z_k\rangle)}\right),
\end{align}
where $\mathbb{E}_{\mathrm{shadow}s~\sigma}[\sigma]=\frac{\langle z_k\vert\rho\vert z_k\rangle}{\mathrm{tr}(\langle z_k\vert\rho\vert z_k\rangle)}$ is a normalized state as discussed in \cite{huang2020predicting} and Appendix B of \cite{huang2024certifying}. This is because shadows of a state average to the unknown state by construction.

The overall variance of $\omega$ therefore is upper bounded by $\mathrm{Var}[\omega]\leq 3.25$. To see this, consider the contribution to variance due to $\omega_{z_k}$ where $\mathbb{E}[\omega]-\mathbb{E}[\omega_{z_k}]=\delta_{z_k}$. Then,
\begin{align}
\mathbb{E}\left[(\omega_{z_k}-\mathbb{E}\left[\omega\right])^2\right]&=\mathbb{E}\left[(\omega_{z_k}-\mathbb{E}\left[\omega_{k_z}\right]+\delta_{z_k})^2\right]\\
&=\mathbb{E}\left[(\omega_{z_k}-\mathbb{E}\left[\omega_{z_k}\right])^2+2(\omega_{z_k}-\mathbb{E}\left[\omega_{z_k}\right])+\delta_{z_k}^2\right]\\
&=\mathrm{Var}\left[\omega_{z_k}\right]+\delta_{z_k}^2.
\end{align}
Note that we have the constraint that $\sum_{z_k}p_{z_k}\cdot\delta_{z_k}=0$ since $\sum_{z_k}p_{z_k}\cdot\mathbb{E}[\omega_{z_k}]=\mathbb{E}[\omega]$, where $p_{z_k}$ is the probability of selecting $m$ random qubits denoted by $k$ and measuring the rest of the $n-m$ qubits output bitstring $z_k$. Further, we have $\delta_{z_k}\in[-\mathbb{E}[\omega], 1-\mathbb{E}[\omega]]$. It is easy to see that the maximum possible value of $\sum_{z_k}p_{z_k}\cdot\delta_{z_k}^2\leq-\mathbb{E}[\omega]\cdot(1-\mathbb{E}[\omega])\leq0.25$, where the equality is satisfied by a distribution where all the probability mass concentrates on the boundary. Therefore,
\begin{align}
\mathrm{Var}[\omega]&=\sum_{z_k}p_{z_k}\cdot\mathbb{E}\left[(\omega_{z_k}-\mathbb{E}\left[\omega\right])^2\right]\leq\sum_{z_k}p_{z_k}\cdot(\mathrm{Var}\left[\omega_{z_k}\right]+\delta_{z_k}^2)\leq3 + \sum_{z_k}p_{z_k}\cdot\delta_{z_k}^2 \leq 3.25.
\end{align}




\parbox{0.96\textwidth}{\begin{protocol_framed}[Improved level-$m$ shadow overlap with random Cliffords]\label{prot:random_clifford_improved}\quad 
\normalfont
\newline
\begin{flushleft}\underline{Input:}\end{flushleft}
 Same as Protocol \ref{prot:random_pauli_improved}.
\begin{flushleft}\underline{Procedure:}\end{flushleft}
All steps are the same as Protocol \ref{prot:random_pauli_improved} except step 3, which we describe here.
For qubits $k_1,\dots,k_m$, generate a circuit $U$ from the $m$ qubit Clifford group $\mathrm{Cl}(2^m)$ uniformly at random and apply it to the $m$ qubits. Then, perform computational basis measurement and record the resulting $m$-bit string $b$. Compute the classical shadow
\begin{align}
    \sigma=(2^m + 1)U^\dagger \vert b\rangle\langle b\vert U-\mathbb{I}.\label{eqn:clifford_shadow}
\end{align}
\end{protocol_framed}}

\begin{lemma}\label{lem:trace_equal_shadow_overlap_clifford}
For $\omega$ of Protocol \ref{prot:random_clifford_improved}, we have
\begin{align}
\mathrm{tr}(L\rho)=\mathbb{E}[\omega].
\end{align}
\end{lemma}
\begin{proof}
The proof is identical to Lemma \ref{lem:trace_equal_shadow_overlap_pauli}. Specifically, the difference between the two proofs only occurs during the step of
\begin{align}
\frac{\langle z_k\vert\rho\vert z_k\rangle}{\mathrm{tr}(\langle z_k\vert\rho\vert z_k\rangle)}=\underset{\mathrm{shadow}s~\sigma}{\mathbb{E}}[\sigma].
\end{align}
In Protocol \ref{prot:random_pauli_improved}, $\sigma$ is a shadow computed from random Pauli measurements according to Eq.~\ref{eqn:pauli_shadow}, and the expectation is over random Pauli basis and measurement outcomes. In Protocol \ref{prot:random_clifford_improved}, $\sigma$ is a shadow computed from random Clifford measurements according to Eq.~\ref{eqn:clifford_shadow}, and the expectation is over random Clifford circuits and measurement outcomes.
\end{proof}

\begin{theorem}\label{thm:shadow_implies_fidelity_clifford}
Theorem \ref{thm:shadow_implies_fidelity_pauli} also holds for $\omega$ as defined in Protocol \ref{prot:random_clifford_improved}.
\end{theorem}
\begin{proof}
The proof is identical to Theorem 4 of \cite{huang2024certifying}.
\end{proof}

\begin{theorem}\label{thm:improved_clifford_sample_complexity_estimator}
Using $T=(\frac{6.5}{\varepsilon^2}+\frac{2}{3\varepsilon}\cdot2^m)\cdot\ln\frac{2}{\delta}$ samples of the state $\rho$, the empirical average $\frac{1}{T}\sum_{t=1}^T\omega_t$ computed by Protocol \ref{prot:random_clifford_improved} is within $\varepsilon$ additive distance from the shadow overlap $\mathbb{E}[\omega]$ with probability at least $1-\delta$.
\end{theorem}
\begin{proof}
We first bound the individual values in the sum.
\begin{align}
\mathrm{tr}(L_{z_k}\sigma)&=\mathrm{tr}\left\{\vert\Psi_{z_k}\rangle\langle\Psi_{z_k}\vert\left[(2^m+1)U^\dagger\vert b\rangle\langle b\vert U-\mathbb{I}\right]\right\}\\
&=(2^m+1)\cdot\vert\langle b\vert U\vert\Psi_{z_k}\rangle\vert^2-1.
\end{align}
Therefore, $-1\leq\mathrm{tr}(L_{z_k}\sigma)\leq2^m$. Further, we know $\mathrm{Var}[\omega]\leq3.25$. By Bernstein's inequality,
\begin{align}
\Pr\left[\left\vert\frac{1}{T}\sum_{t=1}^T\omega_t-\mathbb{E}[\omega]\right\vert>\varepsilon\right]\leq2e^{-\frac{T\varepsilon^2}{2\times 3.25+\frac{2}{3}\times2^m\varepsilon}}\leq\delta.
\end{align}
Solving for $T$ completes the proof.
\end{proof}

\begin{theorem}\label{thm:improved_clifford_sample_complexity_certification}
Given any $n$-qubit hypothesis state $\vert\psi\rangle$ with a relaxation time $\tau\geq 1$, error $\varepsilon>0$, failure probability $\delta>0$, and
\begin{align}
T=\left(\frac{104\tau^2}{\varepsilon^2}+\frac{8\tau}{3\varepsilon}\cdot2^m\right)\cdot\ln\frac{2}{\delta}
\end{align}
samples of an unknown $n$-qubit state $\rho$, with probability at least $1-\delta$, Protocol \ref{prot:random_clifford_improved} with shadow overlap threshold $\omega_{\mathrm{threshold}}\equiv1-\varepsilon'=\frac{3\varepsilon}{4\tau}$ will correctly output \textsc{Failed} if the fidelity is low, i.e. $\langle\psi\vert\rho\vert\psi\rangle<1-\varepsilon$, and will correctly output \textsc{Certified} if the fidelity is high, i.e. $\langle\psi\vert\rho\vert\psi\rangle\geq1-\frac{\varepsilon}{2\tau}$.
\end{theorem}
\begin{proof}
The proof is identical to Theorem 6 of \cite{huang2024certifying} except we use Theorem \ref{thm:improved_clifford_sample_complexity_estimator}. Simply substituting $\varepsilon\rightarrow\varepsilon/\tau-\varepsilon'=\frac{\varepsilon}{4\tau}$ of Theorem 5 of \cite{huang2020predicting} or Theorem \ref{thm:improved_clifford_sample_complexity_estimator} of this work gives the sample complexity of Theorem 6 of \cite{huang2024certifying} or this theorem, respectively.
\end{proof}


We note that there is a substantial improvement in the sample complexity compared to Theorem \ref{thm:random_pauli_verification} for the random Pauli shadow overlap protocol. First, there is an apparent quadratic improvement from $2^{2m}$ to $2^m$. Moreover, the exponential factor in $m$ is additionally improved to proportional to $\frac{\tau}{\varepsilon}$ instead of $(\frac{\tau}{\varepsilon})^2$. The term proportional to $(\frac{\tau}{\varepsilon})^2$ only has a constant factor independent of $m$.

There is also a substantial improvement in sample complexity compared to Theorem \ref{thm:fixed_huang_verification_completeness_and_soundness} for the original shadow overlap protocol of \cite{huang2024certifying}, with a quartic improvement from $2^{4m}$ to $2^m$.

The exponential dependence on $m$ can be further removed by using the median of means estimator, which requires $\frac{64\mathrm{Var}\ln(1/\delta)}{\varepsilon^2}$ samples to estimate the mean of a random variance with error at most $\varepsilon$ and failure probability at most $\delta$. This is exactly as discussed in \cite{huang2020predicting}, and the sample complexity only depends on the variance. The disadvantage of the approach is that is has a large constant factor. Specifically, substituting $\varepsilon\rightarrow\frac{\varepsilon}{4\tau}$ and $\mathrm{Var}=3.25$ yields a sample complexity of $3{,}328\cdot\frac{\tau^2}{\varepsilon^2}\cdot\ln\frac{1}{\delta}$. The advantage of the median of means estimator would only be apparent for large $m$. Under the median of means estimator scheme, the special case of $m=n$ becomes exactly the random Clifford classical shadow approach in \cite{huang2020predicting} for estimating the fidelity.

This makes apparent the fact that our protocol is a unification of the direct classical shadow approach of \cite{huang2020predicting} and the shadow overlap approach of \cite{huang2024certifying} for certifying the quantum state fidelity. On the one extreme, the direct classical shadow approach using random Clifford circuits is sample efficient in that the sample complexity does not increase with $n$, and states fidelities can be estimated in an unbiased manner since the relaxation time $\tau$ is $1$. One can replace random Cliffords with random single-qubit Pauli measurements and the estimator is unbiased since the relaxation time is also 1, but the sample complexity is exponential in $n$. On the other extreme, the shadow overlap approach that measures one random qubit in a random Pauli basis achieves low sample complexity that is independent of $n$, but the relaxation time $\tau$ is large and low fidelity states cannot be \textsc{Certified}.

Our work bridges the gap by introducing a family of protocols that connect the two extremes. We can go from the extreme of large relaxation time to the minimum relaxation time by increasing the level $m$ of the protocol. Additionally, the sample complexity is $O(2^{2m})$ for the random Pauli protocol that preserves the desirable property that the measurement is easy to implement. For the random Clifford protocol, the sample complexity is $O(2^m)$ or independent of $m$ for the mean estimator or the median of means estimator, respectively. The complexity of implementing the measurement, which is $O(m^2)$ since implementing a random Clifford circuit requires quadratically many gates, can be controlled by keeping $m$ moderate.

Although \cite{huang2020predicting} also introduces a family of protocols parameterized by the level $m$, the choice of operator $L$ does not lead to a correspondence with the direct random Clifford classical shadow approach of \cite{huang2020predicting} even when $m=n$, and the relaxation time remains large as $m$ increases. Further, the sample complexity is $O(2^{4m})$, which prohibits practical use for large $m$.

\subsection{Certifying the state in our experiment}\label{sec:supp_cert_experiment}


The sample complexity used in Theorem \ref{thm:improved_clifford_sample_complexity_certification} is for both completeness and soundness. However, once the experimental results on the shadow overlap protocol is collected, one can carry out a hypothesis test to see if the lab state has fidelity at least $1-\varepsilon$ and not worry about the completeness side. This motivates the following corollary.

\begin{corollary}\label{cor:sample_complexity_soundness}
If for $\varepsilon\geq\tau\varepsilon'$, the number of shadows collected by Protocol \ref{prot:random_clifford_improved} is $T\geq(\frac{6.5}{(\varepsilon/\tau-\varepsilon')^2}+\frac{2}{3\times(\varepsilon/\tau-\varepsilon')}\cdot 2^m)\cdot\ln\frac{1}{\delta}$, then either the protocol outputs \textsc{Failed} with probability at least $1-\delta$, or $\langle\psi\vert\rho\vert\psi\rangle\geq1-\varepsilon$.
\end{corollary}
\begin{proof}
If $\langle\psi\vert\rho\vert\psi\rangle<1-\varepsilon$, then $\mathbb{E}[\omega]<1-\varepsilon/\tau$. To pass the protocol, we need $\hat{\omega}-\mathbb{E}[\omega]>\varepsilon/\tau-\varepsilon'$. From the proof of Theorem~\ref{thm:improved_clifford_sample_complexity_estimator}, switching from two-sided to one-sided Bernstein's inequality yields
\begin{align}
\Pr\left[\frac{1}{T}\sum_{t=1}^T\omega_t-\mathbb{E}[\omega]>\varepsilon\right]\leq e^{-\frac{T\varepsilon^2}{2\times 3.25+\frac{2}{3}\times2^m\varepsilon}}.\label{eqn:one_sided_bernstein}
\end{align}
Then, substituting $\varepsilon$ in the Eq.~\ref{eqn:one_sided_bernstein} with $\varepsilon/\tau-\varepsilon'$ shows that the protocol must output \textsc{Failed} with probability at least $1-\delta$.
\end{proof}

For our experiment, we are not in the ideal perfect honest fidelity case, so we need Lemma \ref{lem:depolarizing_noise} to bound the infidelity of the adversary state relative to the laboratory state. Assume that the adversary can prepare a state $\lvert\psi_{\rm{adv}}\rangle$ with fidelity $\vert\langle\psi_{\rm{adv}}|\psi_{\rm{hon}}\rangle\vert^2\leq1-\varepsilon_{\rm{CNL}}=0.01$. Further, we have empirically estimated that the honest lab state infidelity is at least $\varepsilon_{\rm{hon}}\leq0.11$, Lemma \ref{lem:depolarizing_noise} implies that the adversary state fidelity to the lab state is
\begin{align}
\vert\langle0\vert C'^{\dagger}\sigma_{\mathrm{lab}}C'\vert0\rangle\vert^2\leq1-(\varepsilon_{\mathrm{CNL}}-\varepsilon_{\mathrm{hon}})+\varepsilon_{\mathrm{hon}}\frac{1}{2^n}=0.12
\end{align}
under depolarizing noise. Therefore, we set $\varepsilon=1-0.12=0.88$. The shadow overlap test threshold is $\omega_{\mathrm{threshold}}=1-\varepsilon'=0.91$, which means $\varepsilon'=0.09$. Finally, the probability (risk) that a given adversary circuit exceeds the shadow overlap threshold is $\delta$. For this set of parameters, one can achieve $\delta=0.36$ at $T=17{,}316$ samples.

The above corollary cannot guarantee that the state is certified with good security in our particular experiment since $\delta$ is very large. As a result, we use the following result to obtain a tighter bound, which allows us to go to as low as $\delta=0.15$.

\ml{@Akshay to fill out details.}

\begin{theorem}\label{thm:unpublished}
The procedure described in Ref.~\cite{zhang2026efficient} takes as input the list of $T$ measured observer values $\{\omega_i\}_{i\in[T]}$, lower and upper bounds for $\omega_{\mathrm{min}}\leq\omega_i\leq \omega_{\mathrm{max}}$ for all $i\in[T]$, a confidence/security parameter $\delta$, and outputs an lower bound $b(T, \delta,\omega_{\mathrm{max}}, \omega_{\mathrm{min}},\{\omega_i\}_{i\in[T]})$ such that
\begin{align}
\underset{\{\omega_i\}_{i\in[T]}}{\Pr}[\mathbb{E}[\omega]<b(T, \delta,\omega_{\mathrm{max}}, \omega_{\mathrm{min}},\{\omega_i\}_{i\in[T]})]<\delta
\end{align}
\end{theorem}

Theorem~\ref{thm:unpublished} is essentially the counter part of Theorem~\ref{thm:improved_clifford_sample_complexity_estimator} except no explicit analytical bound is given. To see this connection more clearly, one can rephrase Theorem~\ref{thm:improved_clifford_sample_complexity_estimator} as a special case of Theorem~\ref{thm:unpublished} with
\begin{align}
b(T, \delta,\omega_{\mathrm{max}}, \omega_{\mathrm{min}},\{\omega_i\}_{i\in[T]})=\frac{1}{T}\sum_{t=1}^T\omega_t+\varepsilon,
\end{align}
where $\varepsilon$ can be obtaining by solving the following equality using the quadratic formula:
\begin{align}
e^{-\frac{T\varepsilon^2}{2\times 3.25+\frac{2}{3}\times2^m\varepsilon}}=\delta,
\end{align}
which comes from switching from two-sided to one-sided Bernstein's inequality just as in Corollary~\ref{cor:sample_complexity_soundness}.

Of course, phrased in this way, Protocol
~\ref{prot:random_clifford_improved} is no longer well defined, since we are only given access to the lower bound $b$ and not the estimator $\hat{\omega}$ anymore, which is needed in step 7 when determining whether to output \textsc{Certified} or \textsc{Failed}. Instead, we define the following protocol.

\parbox{0.96\textwidth}{\begin{protocol_framed}[Improved level-$m$ shadow overlap with random Cliffords]\label{prot:using_lower_bound_procedure}\quad 
\normalfont
\newline
\begin{flushleft}\underline{Input:}\end{flushleft}
 Same as Protocol \ref{prot:random_clifford_improved}.
\begin{flushleft}\underline{Procedure:}\end{flushleft}
All steps are the same as Protocol \ref{prot:random_clifford_improved} except step 6 and 7, which we describe here.

For step 6, compute the lower bound $b(T, \delta,\omega_{\mathrm{max}}, \omega_{\mathrm{min}},\{\omega_i\}_{i\in[T]})$.

For step 7, if $b\geq 1-\varepsilon'$, output \textsc{Certified}. Otherwise, output \textsc{Failed}.

\end{protocol_framed}}

It should be noted that in Protocol~\ref{prot:random_clifford_improved}, $\omega_{\mathrm{threshold}}=1-\varepsilon'$ is set such that it is slightly above the expected shadow overlap of the adversarial case $\mathbb{E}[\omega_{\mathrm{adv}}]$. This is to allow for some fluctuations in the empirical estimator $\hat{\omega}$. On the other hand, for Protocol~\ref{prot:using_lower_bound_procedure}, the lower bound $b$ is already estimated to allow for statistical fluctuations due to the samples, so $\omega_{\mathrm{threshold}}=1-\varepsilon'$ should be set to exactly $\mathbb{E}[\omega_{\mathrm{adv}}]$.











